Findings of the Second BabyLM Challenge: Sample-Efficient Pretraining on Developmentally Plausible Corpora

The BabyLM Challenge is a community effort to close the data-efficiency gap between human and computational language learners. Participants compete to optimize language model training on a fixed language data budget of 100 million words or less. This year, we released improved text corpora, as well as a vision-and-language corpus to facilitate research into cognitively plausible vision language models. Submissions were compared on evaluation tasks targeting grammatical ability, (visual) question answering, pragmatic abilities, and grounding, among other abilities. Participants could submit to a 10M-word text-only track, a 100M-word text-only track, and/or a 100M-word and image multimodal track. From 31 submissions employing diverse methods, a hybrid causal-masked language model architecture outperformed other approaches. No submissions outperformed the baselines in the multimodal track. In follow-up analyses, we found a strong relationship between training FLOPs and average performance across tasks, and that the best-performing submissions proposed changes to the training data, training objective, and model architecture. This year's BabyLM Challenge shows that there is still significant room for innovation in this setting, in particular for image-text modeling, but community-driven research can yield actionable insights about effective strategies for small-scale language modeling.

==> tables/aoa.tex <==
\resizebox{\textwidth}{!}{%
    \begin{tabular}{clrrrr}
    \toprule
        & \multirow{2}{}{\textbf{Model}} & \multicolumn{4}{c}{\bf Mean average deviation $\downarrow$}\\
        
        & & \bf Overall & \bf Nouns &\bf Predicates & \bf  Function Words \\
    \midrule
     % \cline{3-6}
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{Strict}}}} & BabyStories (GPT2-Large-PPO)~\cite{babylm2023babystories} & 2.05 & 1.98 & \underline{\textbf{1.82}} & 2.63 \\
         & \emph{Best Baseline (OPT-125M)} & \underline{\textbf{2.04}} & \underline{\textbf{1.97}} & 1.83 & \underline{\textbf{2.61}} \\
    \midrule
        \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small{Strict-Small}}}}  & GPT-Wee (16k (cu.))~\citep{babylm2023gptwee} & 2.06 & 2.00 & 1.83 & 2.58 \\
         & Bebeshka \citep{babylm2023miniminds} & 2.06 & 1.98 & 1.84 & 2.66 \\
         & Zlata \citep{babylm2023miniminds} & 2.07 & 1.99 & 1.83 & 2.67 \\
         & Too Much Information \citep{babylm2023toomuch} & 2.05 & 1.99 & 1.85 & 2.58 \\
         & Mmi01 (\textsc{Rarity})~\cite{babylm2023mmi01} & 2.05 & \underline{\textbf{1.97}} & 1.85 & 2.64 \\
         & Baby Llama~\citep{babylm2023babyllama} & 2.06 & 1.99 & 1.84 & 2.63 \\
         & Lil-Bevo-X~\citep{babylm2023lilbevo} & 2.05 & 1.99 & 1.85 & 2.59 \\
         & \emph{Best Baseline (OPT-125M)} & \underline{\textbf{2.03}} & 1.98 & \underline{\textbf{1.81}} & \underline{\textbf{2.57}} \\
         %& &  &  &  &  & \\\\
    \bottomrule
    \end{tabular}
    }
    \captionof{table}{Mean average deviation (MAD) in months across cross-validation folds when predicting the age of acquisition of words. Lower MAD scores are better. We present all systems that evaluated on AoA prediction, as well as the baseline model with the best scores per track. We \underline{\textbf{bold}} the highest-scoring system for each task within each track.}
% \end{minipage}
\label{tab:aoa_eval}

==> tables/hypernym.tex <==
% \begin{table*}[phtb]
\begin{tabular}{>{\hangindent=2em}p{0.3\textwidth}>{\hangindent=1em}p{0.3\textwidth} >{\hangindent=1em}p{0.32\textwidth}}
\toprule
    \bf Contrast name & \bf Acceptable sentence & \bf Unacceptable sentence\\
\midrule
    
    \small\contrast{base\_and\_hyponym/ hypernym} & If he is growing herbs, then he is growing plants. & If he is growing herbs, then he is growing basil.\\
    
    \small\contrast{base\_neg\_and\_hypernym\_neg/ converse} & If he isn't growing herbs, that means he isn't growing basil. & If he isn't growing basil, that means he isn't growing herbs.\\
    
    \small\contrast{base\_neg\_and\_hypernym\_neg/ hyponym\_neg} & If he isn't growing herbs, that means he isn't growing basil. & If he isn't growing herbs, that means he isn't growing plants.\\
    
    \small\contrast{hypernym\_and\_base/ converse} & If he is growing basil, that means he is growing herbs. & If he is growing herbs, that means he is growing basil.\\
    
    \small\contrast{hypernym\_and\_base/ other} & If he is growing basil, then he is growing herbs & If he is growing basil, then he is growing flowers.\\
    \small\contrast{hypernym\_and\_other\_neg/ base\_neg} & He is growing basil, therefore he isn't growing flowers. & He is growing basil, therefore he isn't growing herbs.\\
\bottomrule
\end{tabular}
\captionof{table}{Representative examples from the \testsuite{Hypernyms} test suite of the BLiMP supplement.}
\label{tab:hypernym}
% \end{table*}

==> tables/msgs.tex <==
% \resizebox{\texwidth}{!}{%
\begin{tabular}{lllllllll}
    \toprule
        \textbf{} & \textbf{ Model} & 
        \msgstask{Macro Avg.} & 
        \msgstask{Ctl--Raising /\\Lexical content} & 
        \msgstask{Ctl--Raising /\\Relative position} & 
        \msgstask{Main verb /\\Lexical content} & 
        \msgstask{Main verb /\\Relative position} & 
        \msgstask{Syntactic cat. /\\Lexical content} & 
        \msgstask{Syntactic cat. /\\Relative position} \\ 
    \midrule
        ~ & LLaMA 2 \citep{llama2} & -0.249 & \-0.939 & \-0.238 & -0.775 & -0.964 & -0.192 & -0.743 \\ 
        ~ & RoBERTa-base \citep{liu-etal-2019-roberta} & -0.370 & \-0.469 & -0.584 & -0.955 & -0.942 & \-0.360 & -0.573 \\ 
    \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small{Strict}}}} 
        & ELC-BERT \citep{babylm2023notall} & \-0.104 & -0.518 & -0.460 & \-0.711 & \-0.974 & \-0.461 & -0.538 \\ 
        ~ & Boot-BERT \citep{babylm2023meanberts} & -0.226 & \-0.377 & -0.776 & -0.996 & \-0.966 & -0.342 & -0.586 \\ 
        ~ & McGill \citep{babylm2023mcgill} & -0.351 & \-0.651 & -0.700 & -0.999 & -0.737 & \-0.170 & -0.493 \\ 
        ~ & \emph{Best Baseline (OPT-125M)} & -0.393 & \-0.354 & -0.703 & -0.761 & -0.995 & \-0.346 & -0.604 \\ 
    \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small{Strict-small}}}} 
        & ELC-BERT \citep{babylm2023notall} & -0.014 & \-0.027 & -0.715 & \-0.955 & \-0.503 & -0.265 & -0.592 \\ 
        ~ & MLSM \citep{babylm2023cogmemlm} & -0.370 & \-0.316 & -0.566 & -0.996 & -0.494 & -0.033 & -0.447 \\ 
        ~ & McGill \citep{babylm2023mcgill} & -0.605 & -0.681 & -0.379 & -1 & -0.794 & -0.355 & -0.422 \\ 
        ~ & \emph{Best Baseline (OPT-125M)} & -0.458 & \-0.003 & -0.703 & -0.721 & -0.775 & \-0.137 & -0.689 \\ 
    \midrule
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\small{Loose}}}} 
        & Contextualizer \citep{babylm2023contextualizer} & \-0.241 & \-0.880 & \-0.717 & -0.320 & \-0.309 & \-0.219 & -0.359 \\ 
        ~ & McGill \citep{babylm2023mcgill} & -0.755 & -0.568 & -0.971 & -0.990 & -0.864 & -0.669 & -0.468 \\ 
        ~ & BabyStories \citep{babylm2023babystories} & -0.710 & -0.246 & -0.992 & -0.997 & -0.994 & -0.239 & -0.789 \\ 
    \bottomrule
\end{tabular}
% }
\captionof{table}{MSGS results by subtask for the top performing models (by overall score) from each track, as well as baselines and skylines.}
\label{tab:msgs_subtasks}

==> tables/qa_congruence.tex <==
% \begin{table*}[t]
    % \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll>{\hangindent=1em}p{0.39\textwidth} >{\hangindent=1em}p{0.39\textwidth}}
    \toprule
        \bf Contrast name & \bf Dif. & \bf Acceptable dialogue & \bf Unacceptable dialogue\\\midrule
        \small\contrast{animate vs. inanimate} & easy & A: What did you purchase?\n~B: Bread. & A: What did you purchase?\n~B: David.\\
        \small\contrast{inanimate vs. animate} & easy & ``Who played the piano?" he asked. ``A teacher played the piano," she said. & ``Who played the piano?" he asked. ``A car played the piano," she said.\\
        \small\contrast{loc vs. NP} & easy & David: Where did you put it?\n~Sarah: Behind the sofa. & David: Where did you put it?\n~ Sarah: Eggs. \\
        \small\contrast{animate vs. inanimate} & tricky & David: Who mopped?\n~Sarah: A doctor. & David: Who mopped?\n~Sarah: The tiles. \\
        \small\contrast{loc vs. NP} & tricky & A: Where were you reading?\n~B: By the lake. & A: Where were you reading?\n~B: An essay.\\
        \small\contrast{temp vs. NP} & tricky & When did you eat?\n~Several minutes ago. & When did you eat?\n~Dinner. \\
        \small\contrast{expl vs. NP} & tricky & ``Why were you reading?" he asked. ``For fun," she said. & ``Why were you reading?" he asked. ``A book," she said. \\
        \small\contrast{num vs. NP} & tricky & A: How many do you teach?\n~B: A few. & A: How many do you teach?\n~B: History. \\
        \small\contrast{manner vs. NP} & tricky & David: How did you vacuum?\n~Sarah: I vacuumed quickly. & David: How did you vacuum?\n~Sarah: I vacuumed the patio. \\
        
    \bottomrule
    \end{tabular}
    }
    \captionof{table}{Representative examples from the \testsuite{Question-Answer Congruence} test suite of the BLiMP supplement.}
    \label{tab:turntaking2}
% \end{table*}


==> tables/result_table.tex <==
\begin{table*}[tbhp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{clrrrrr}
    \toprule 
        & \textbf{Model} & BLiMP & GLUE & MSGS & BLiMP-Supp. & \emph{Aggregated}\\
    \hline
        %\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{Pretrained}}}} & Llama 2 &  &  &  &  & \\
         & Llama 2 & 0.84 & 0.84 & 0.26 & 0.75 & 0.71 \\
         & RoBERTa-Base & 0.87 & 0.79 & 0.24 & 0.76 & 0.70 \\
    \hline
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small{Strict}}}} & ELC-BERT~\cite{babylm2023notall} & 0.85 & 0.78 & \underline{\textbf{0.47}} & \underline{\textbf{0.77}} & \underline{\textbf{0.74}} \\
         & BootBERT~\cite{babylm2023meanberts} & \underline{\textbf{0.86}} & \underline{\textbf{0.79}} & 0.28 & 0.72 & 0.70 \\
         & McGill-BERT~\cite{babylm2023mcgill} & 0.84 & 0.72 & 0.25 & 0.71 & 0.67 \\ % do we have an official name for some model?
         & \emph{Best Baseline (OPT-125M)} & 0.75 & 0.70 & 0.13 & 0.68 & 0.60 \\
         %& \emph{RoBERTa-Base-Baseline} & 0.50 & 0.71 & 0.04 & 0.42 & 0.46 \\
    \hline
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small{Strict-Small}}}} & ELC-BERT~\cite{babylm2023notall} & \underline{\textbf{0.80}} & \underline{\textbf{0.74}} & \underline{\textbf{0.29}} & 0.67 & \underline{\textbf{0.66}} \\
         & MLSM~\cite{babylm2023bettertogether} & 0.79 & 0.71 & 0.17 & 0.57 & 0.61 \\
         & McGill-BERT~\cite{babylm2023mcgill} & 0.75 & 0.70 & 0.13 & \underline{\textbf{0.68}} & 0.60 \\
         & \emph{Best Baseline (OPT-125M)} & 0.63 & 0.62 & 0.10 & 0.53 & 0.50 \\
         %& &  &  &  &  & \\
    \hline
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\small{Loose}}}} & Contextualizer~\cite{babylm2023contextualizer} & \underline{\textbf{0.86}} & \underline{\textbf{0.73}} & \underline{\textbf{0.58}} & 0.63 & \underline{\textbf{0.73}} \\
         & McGill-BERT~\cite{babylm2023mcgill} & 0.80 & 0.68 & -0.02 & 0.57 & 0.57 \\
         & BabyStories~\cite{babylm2023babystories} & 0.78 & 0.61 & 0.03 & \underline{\textbf{0.65}} & 0.56 \\
    \bottomrule
    \end{tabular}}
    \caption{Top 3 systems for each track, as well as the baseline model with the highest aggregate score. We also show ``skyline'' models: RoBERTa-base and Llama 2 trained on their full pre-training corpora. Each task score is simply the mean score across each of its subtasks. The aggregate score is a weighted average of each task. We \underline{\textbf{bold}} the highest-scoring system for each task within each track.}
    \label{tab:result}
\end{table*}

==> tables/turn_taking.tex <==
% \begin{table*}[t]
    % \centering
    \begin{tabular}{ll>{\hangindent=1em}p{0.37\textwidth} >{\hangindent=1em}p{0.37\textwidth}}
    \toprule
        \bf Type & \bf Length & \bf Acceptable dialogue & \bf Unacceptable dialogue\\\midrule
        single & short & David: Should you quit?\textbackslash n Sarah: No, I shouldn't. & David: Should she quit?\textbackslash n Sarah: No, I shouldn't. \\
        single & long & Did they try to finish it on time or not?\textbackslash n No, they didn't. & Did we try to finish it on time or not?\textbackslash n No, they didn't.\\
        double & short & A: Did we say that you finished?\textbackslash n B: Yes, you did. & A: Did you say that you finished?\textbackslash n B: Yes, you did.\\
        double & long & ``Did you say that you will go somewhere after the movie is over?" he asked.\textbackslash n ``No, I didn't," she said.  & ``Did you say that you will go somewhere after the movie is over?" he asked.\textbackslash n ``No, you didn't," she said.\\
    \bottomrule
    \end{tabular}
    \captionof{table}{Representative examples from the \testsuite{Turn-Taking} test suite of the BLiMP supplement.}
    \label{tab:turntaking1}
% \end{table*}

